GraspLook: a VR-based Telemanipulation System with R-CNN-driven Augmentation of Virtual Environment

The teleoperation of robotic systems in medical applications requires stable and convenient visual feedback for the operator. The most accessible approach to delivering visual information from the remote area is using cameras to transmit a video stream from the environment. However, such systems are sensitive to the camera resolution, limited viewpoints, and cluttered environment bringing additional mental demands to the human operator. The paper proposes a novel system of teleoperation based on an augmented virtual environment (VE). The region-based convolutional neural network (R-CNN) is applied to detect the laboratory instrument and estimate its position in the remote environment to display further its digital twin in the VE, which is necessary for dexterous telemanipulation. The experimental results revealed that the developed system allows users to operate the robot smoother, which leads to a decrease in task execution time when manipulating test tubes. In addition, the participants evaluated the developed system as less mentally demanding (by 11%) and requiring less effort (by 16%) to accomplish the task than the camera-based teleoperation approach and highly assessed their performance in the augmented VE. The proposed technology can be potentially applied for conducting laboratory tests in remote areas when operating with infectious and poisonous reagents.

==> Last_paper_comments.tex <==

Related works


%A number of researchers are trying to combine kinesthetic feedback with force feedback by using tactile display \cite{10.1007/978-3-642-31401-8_34}. They presented an experiment of two-finger grasping. The task considered was the peg-in-hole and the simulated force feedback is cutaneous or kinesthetic. The kinesthetic feedback was provided by a commercial haptic device while the cutaneous one is provided by a new haptic display proposed in this research. This work in many aspects motivated our own work. Also one of the good solutions can be using of electrotactile displays.

 %Electrotactile stimulation, also known as electrocutaneous,  allows to educe tactile or touch sensation within the skin by passing an electric current through the skin at the location of the electrode. It can evoke a range of sensations, including tingling, itching, vibration, pinch, pressure, or touch.


%=======================================================
% \section{Material and software}
% In this section we describe the control of the robot-manipulator and the mechanism of the electotactile sensors.


\subsection{Universal Robot UR3}
% The robotic manipulator used in this project is Universal Robot UR3, shown in % link to the image
% . This's is smallest UR robot which has 6 degree of freedom (DoF), weights 11kg, with a payload of 3 kg and horizontal reach 500mm, repeatability $\pm{0.1}$ mm. The UR3 can provide the enough accuracy and agility to many applications. 

% \subsection{ROBOTIQ 2F-85 gripper}
% % Description of the electrotactile sensors and electrodes, gripper, force sensor.
% For the project we use the ROBOTIQ 2F-85 gripper, which can be controlled by closing distance (from 0 to 85 mm), closing speed (from 20 to 150 mm/s), grip force (from 20 to 235 N). This device weights 0.9 kg, and can lift max 5 kg of payload. On the gripper fingers the electotactile sensors attached to provide the information about contact area. 

% \subsection{Electro-stimulation system}
% % Jonathan please describe the part about your sensors, and why we're using the force sensor with the gripper 

% \subsection{Force Dimension Omega 7 haptic device}
% The Force Dimension Omega 7 is a haptic device which uses for the most advanced multiple point-of-contact touch-enabled applications. With a delta base parallel kinematics, the device provides electromagnetic feedback, has \oslash $160 \times 110$ mm translation, 
% $240 \times 140 \times 180$ deg rotation and 25 mm grasping. The device has 4 active and 3 passive DoF, the resolution of this device is for translation $< 0.01$ mm, for rotation 0.09 deg, for grasping 0.006 mm which allows to apply this device for even medical applications. Force Dimension products can be used with the haptic and robotc SDK software which use the C++ programming language. 

% \subsection{Unity}
% % ref
% Unity is a cross-platform engine developed by Unity Technologies.The programming language is C\# . It allows to create a scene in virtual environment to simulate various processes. One of the main advantages of it is that it has an advanced physical engine, that allows to calculate object collisions, as well as the ability to connect external devices and the availability of a large number of additional plug-ins. In our case it was used to create a digital twin and to establish communication between all subsystems. Digital twin represents current position of UR3 robot and allows to control it in real time via socket communication. Thrue Unity operator could have real-time visual feedback to control the robot.
% %Implementation of digital twin provides /Description of the digital twin, limitation, environment, collision avoidance.
% %Alexey and Artem, please, fill this part (in general). The control of the system is in next section







 System overview

% The teleportation of the robot manipulator allows the operator to work in the remote or dangerous environment with human precision using the haptic device. The operator controls the position of the robot by the related position of the joystick, the frames of joystick and robot is shown in Fig.  \ref{fig:JoystickFrames}.




%To achieve required position as an input data, the teleoperation control gets three coordinates and three angles of an end-effector. To get the real-time solution for all joints close form solution was used. This method allows to reduce the dimension of the transition matrix, which allows to get a solution for the robot quickly enough for real-time remote control.

%With this approach, we get eight possible solutions. Among the solutions obtained, those that lead the robot to the singularity state are eliminated. As a criterion for choosing a final solution, a link-weighted solution with the lowest weight is selected. This allows to achieve greater smoothness in the robot's movements and avoid it falling into critical positions.

% \begin{figure}[h!]
%   \centering
%   \includegraphics[width=0.47\textwidth]{pictures/inverseKinematics2.png}
%   \qquad
%   \caption{The 5th (a), 7th (b) and 3rd (c) solutions of the the same IK problem during teleoperation task. The virtual famework provides the selection of optimal joint angles.}
%   \label{fig:ikSol}
% \end{figure}
%For this project, it was decided to use sockets as the main method of communication between subsystems. Sockets allow to exchange information between the server and the client in the real-time with minimal delays.

%Coordinates and angles from joystick are send to the digital twin in Unity through the Sockets. the Unity system creates the packet of data with command to the real robot manipulator and send it, the robot moves to the obtained coordinates with defined velocity. For the object grasp the operator close the gripper on the joystick with electrodes, the command about it is also sent to the digital twin, and Unity sends the command to the real manipulator, which has additional electrotactile and force/torque sensors in order to provide the precise data about contact surface. .



% % change the pic on the created by the computer one
% \begin{figure}[h!]
%   \centering
%   \includegraphics[width=0.47\textwidth]{pictures/teleoperation.jpg}
%   \qquad
%   \caption{The joystick and robot's frames.}
%   \label{fig:JoystickFrames}
% \end{figure}


%\subsection{Socken communication}
%Sockets w


% \begin{figure}[h!]
%   \centering
%   \includegraphics[width=0.47\textwidth]{pictures/system.jpg}
%   \qquad
%   \caption{The scheme of the system.}
%   \label{fig:system}
% \end{figure}


% \subsection{Haptic device control}
% In the final version, it was decided that the digital twin and the robot will be controlled by moving. For this purpose, the scales were selected separately for each axis and the angle of rotation of the joystick to cover the maximum working area of the robot.


%============================================




% \begin{figure*}[h!]
%   \centering
%   \includegraphics[width=1 \textwidth, height=19cm]{pictures/graph.png}
%   \qquad
%   \caption{The results of experiment. }
%   \label{fig:results1}
% \end{figure*}

% \section{Discussion}\label{discussion}
% % Discussion of result (what is good/bad, why).
% The experimental results suggested that the simultaneous use of kinesthetic and electrotactile feedback allows to improve the speed and accuracy of the operation with each of the materials under study.

%We suppose that the combination of two feedbacks allows operator to perform with to manage with more flexibility and increase the speed of the operation.
%%=============================================================

%Three steps of the experiment were conducted. During all steps of the experiment, the operator has visual feedback from the manipulator via camera and visual feedback of a digital twin. In each iteration the operator had to take the object from the starting position, move it to the goal position and release it. Two metrics were implied to evaluate the performance of this task: the overclosing rate of the gripper and the time required to perform the task. At the first step the operator has only visual feedback on how much the gripper was opened and whether the object was already captured. 
%During the second step a force feedback was also added. Since only force must be applied at this stage, the value of this force for each finger was calculated as an average for all cells of one finger. Due to the limitations of the joystick does not allow to apply feedback on both sides for the gripper so the average value for two fingers was taken. 
%At the third step  we combined force and kinesthetic feedback. Values from each cell of the sensor were read separately. 

%The experiment was performed with three objects of different shapes and materials. As the first and the second objects, two different balls were chosen: the flexible ball made from elastic rubber 48 mm in diameter and as a second object the tennis ball 60  mm in diameter was used. The third object is a hollow plastic object with cylindrical shape 65 mm in diameter. As it was fragile we decided to add the elastic ball inside to avoid destruction of the object. Models of objects are shown in Fig( \ref{fig:Objects}).
%\begin{figure}[h!]
%  \centering
%  \includegraphics[width=0.48\textwidth]{pictures/3d_objects.png}
%  \caption{  (a) Elastic spherical object 48 mm in diameter. (b)  Hard spherical object 60  mm in diameter. (c) Hollow cylindrical object 65 mm in diameter.}
%  \label{fig:Objects}
%\end{figure}


%\begin{figure}[h!]
%  \centering
%  \includegraphics[width=0.48\textwidth]{pictures/Real_Objects.png}
%  \caption{  (a) Elastic spherical object 48 mm in diameter. (b)  Hard spherical object 60  mm in diameter. (c) Hollow cylindrical object 65 mm in diameter.}
%  \label{fig:Objects}
%\end{figure}

%We conducted nine tests, three per object. All of them were  carried out by right handed person. During the experiment, information about the position of the end-effector was recorded, real information obtained from the robot, and coordinates from Unity. Also recorded information about the state of the gripper as well as their two sources: from the gripper and the joystick, which was controlled. 


\section{Experimental results}





% \begin{figure}[H]
%   \centering
%   \includegraphics[width=0.5\textwidth]{pictures/graph.png}
%   \qquad
%   \caption{Layout of the collaborative robotic system joinTbot.}
%   \label{fig:SystemOverview}
% \end{figure}
\subsection{Visual channel}

%The results of the experiments with three different objects for visual channels are shown in Fig.\ref{fig:visual}. The columns correspond to objects and the rows for 1) comparison the difference between the gripper fingers sent and read positions, 2) data from the pressure sensors on the gripper fingers. The orange line shows the real position of the gripper fingers which we read from the gripper, the green line is the gripper position which we send from the Omega 7 haptic device, the light-green area is the difference between these two positions. The non-zero values of the blue line in the plot with the data from the pressure sensors show the time when the gripper fingers connect with the object. 

%As the first object, the elastic ball was chosen. In an attempt to grasp the ball, the operator has closed the gripper with more than 70 \% overshooting than it was necessary to grasp the object. The red markers show the initial position of the gripper fingers at (8.5 cm) and the minimal position at which the gripper had stopped while squeezing the object. 

%For the second object which is more rigid than the first one, the operator grasps the object with more than 60 \% of overclosing because visual feedback allows the operator to see that the object is in the gripper fingers and fixed there. The projection from the corresponded pressure sensor data on the blue line demonstrates that in moments when the object becomes within the gripper fingers the real position of the gripper fingers (orange line) had become stable, it means that the object didn't deform.

%The third object which is the fragile cylinder the operator grasps the object with more than 30 \% of overclosing. This small percentage is due to the object's susceptibility to shape change (it follows from the fact the orange line didn't become stable) and the object could be breaking with overclosing more than 40 \%. Due to small force applied for grasping this object, the object turned in the gripper fingers and tried to slide out from fingers, the corresponded blue line shows that the pressure sensors detected the moment when the contact with the object quality contact with the object decreased and increased. 

\subsection{Kinesthetic channel}

% \begin{figure*}[h!]
%   \centering
%   \includegraphics[width=\textwidth]{pictures/kinesthetic1.png}
% %   \qquad
%   \caption{The results of experiment for kinesthetic channel. }
%   \label{fig:kinesthetic}
% \end{figure*}

%The results of the experiment with the same three objects for kinesthetic channel where the force feedback was added on the haptic device, is shown in Fig. \ref{fig:kinesthetic}. The purple area on the plots in the second row shows the applied force on the haptic tactile device. 

%The force feedback for the first object on the haptic device allows the operator to decrease the applied force for grasping therefore the difference between the real position of the gripper fingers and the send position from the haptic device is less than for the visual channel on 40 \% of overclosing. The force feedback calculated using the data of positions of grippers finger and the data from the pressure sensors, where the difference between position is the input error for the PID controller of the force feedback.

%For the second object, the force feedback on the Omega 7 device forces the operator to stop the closing of the gripper and the maximum difference between sent and read positions of the gripper fingers is decreased the overclosing of the gripper up to 40 \%. The moment when the force reached the maximum in 3 $N$ forces the operator to decrease the compression of the object which follows from the green line after the 15th second. 

%The force feedback for the third object on the haptic device helps the operator to grasp the object and decrease the overclosing of more than 15 \%. The corresponded plot with data from pressure sensors and applied force demonstrates that the force feedback is adaptive to the changes in the distances of the gripper fingers and the object between them because when the operator is opening the gripper or the objects is turning between fingers, the force feedback is decreased.
\subsection{Tactile channel}

% \begin{figure*}[h!]
%   \centering
%   \includegraphics[width=\textwidth]{pictures/tactile1.png}
% %   \qquad
%   \caption{The results of experiment for tactile channel. }
%   \label{fig:tactile}
% \end{figure*}

%f the experiment with the same three objects and force feedback for tactile channel where the electrodes provide to the operator the shape of the object during the grasping, is shown in Fig. \ref{fig:tactile}.

%For the first object the force feedback with the tactile feedback decreased the time by 1 s for grasping which could be measured by red markers on the plots of gripper positions and the overclosing more than 4 \%. Due to the smaller difference between the gripper positions in comparison with the kinesthetic channel the force feedback applied weaker effect on the operator through the haptic device. In the Fig. \ref{fig:1st} the contact shape from the electrotactile sensors is shown.


The combination of force feedback and the tactile feedback for the second object brings the improvement in time to grasp the object which decreased on 1 s and the overclosing on 15 \% of the gripper fingers. The distance during the holding of the object stays almost stable which is also could be seen on the force feedback curve which is keeping the same values. The contact shape from the electrotactile sensors is shown in Fig. \ref{fig:2nd}.

\begin{figure}[h!]
  \centering
  \includegraphics[width=0.3\textwidth]{pictures/surface_2.png}
  \qquad
  \caption{3D shape of the contact area with the solid sphere.}
  \label{fig:2nd}
\end{figure}

For the third object the tactile feedback and force feedback improved the sensing of the object for the operator therefore the time of the grasping the object decreased on 3 seconds and the overclosing decreased on 10 \%. Due to the real and the sent positions of gripper fingers are close to each other the applied force is weaker in comparison with kinesthetic channel (Fig.\ref{fig:3rd}).
